Synthesizing Formal Semantics from Executable Interpreters

Program verification and synthesis frameworks that allow one to customize the language in which one is interested typically require the user to provide a formally defined semantics for the language. Because writing a formal semantics can be a daunting and error-prone task, this requirement stands in the way of such frameworks being adopted by non-expert users. We present an algorithm that can automatically synthesize inductively defined syntax-directed semantics when given (i) a grammar describing the syntax of a language and (ii) an executable (closed-box) interpreter for computing the semantics of programs in the language of the grammar. Our algorithm synthesizes the semantics in the form of Constrained-Horn Clauses (CHCs), a natural, extensible, and formal logical framework for specifying inductively defined relations that has recently received widespread adoption in program verification and synthesis. The key innovation of our synthesis algorithm is a Counterexample-Guided Synthesis (CEGIS) approach that breaks the hard problem of synthesizing a set of constrained Horn clauses into small, tractable expression-synthesis problems that can be dispatched to existing SyGuS synthesizers. Our tool Synantic synthesized inductively-defined formal semantics from 14 interpreters for languages used in program-synthesis applications. When synthesizing formal semantics for one of our benchmarks, Synantic unveiled an inconsistency in the semantics computed by the interpreter for a language of regular expressions; fixing the inconsistency resulted in a more efficient semantics and, for some cases, in a 1.2x speedup for a synthesizer solving synthesis problems over such a language.

==> algorithms/approx.tex <==
\begin{algorithm}
\Proc{$\algApproxSummary(\mathit{prod}, \mathit{perm}, t, \mathit{SummarySet}, \mathit{synthesizingRec}, \mathit{underapprox}=\bot)$}{

  $(A \mapsto \sigma(A_1,A_2,\dots,A_k)) \gets prod$\;

  $r \gets \top$\;
  \For{$i \in \mathit{perm}(1 \dots k+1)$}{
  
    \lIf{$\overline{\mathit{perm}}(i) = k+1 \land \lnot(\mathit{recursive}(prod) \land synthesizingRec)$}{
        \Break
    }
    $f \gets \top$\;
    \For{$(\mathit{in}, \mathit{out}) \in \mathit{SummarySet}(t, i)$}{
        $f \gets f \land ({x_i^t} = \mathit{in}' \to y_i^t =    \mathit{out})$
        % \lIf{$\lnot \mathit{underapprox}$}{        $f \gets f \land ({x_i^t} = \mathit{in}' \to y_i^t = \mathit{out})$}
        % \lElse{$f \gets f \lor ({x_i^t} = \mathit{in}' \land y_i^t = \mathit{out})$}
    }
    $r \gets r \land f$\;
  }
  \Return{$r$}
}
\caption{Approximate behavior of a child term with a summary set}
\label{alg:approx-summary}
\end{algorithm}

==> algorithms/init-sem.tex <==

\begin{algorithm}
\Proc{$\algInitSem(\mathit{prod}, \mathit{perm}, t, \mathit{in}, \mathit{SummarySet}, \mathit{synthesizingRec})$}{
  % TODO: enumerating weak topological order?
  % TODO: Maybe this is not needed at all! Return a \top will also work! (talk with Charlie)
  $(A \mapsto \sigma(A_1,A_2,\dots,A_k)) \gets prod$\;
  $\Pi \gets \{\text{all components of vector }\mathit{in}\}$\tcp*{all possible semantic inputs}
  $\mathit{SummarySet}' \gets \mathit{SummarySet}$\;
  \For{$i \in \mathit{perm}(1 \dots k+1)$}{
    \uIf{$\overline{\mathit{perm}}(i) = k+1$}{
      \tcp{Even for recursive semantics, there exists a recursive rule and a non-recursive rule. We only continue for the recursive rule.}
      \lIf{$\lnot synthesizingRec$}{\Break}
      \lElse{$t' \gets t$}
    }
    \uElse{
      $t' \gets \text{the $i$-th child term of $t$}$\;
    }
    \tcp{${x_{k+1}}, y_{k+1}$ are I/O vars for recursive call $\semanticBrackets{t'}_{A}$}
    $l \gets \text{dimension count of vector ${x_i}$}$\;
    $Ex \gets \{{x_k} \mid ({x_k}, y_k) \in \mathit{SummarySet}(t, i)\}$\;
    \For{$\mathit{in}' \in Ex \cup (2^{\Pi} \cap \{\text{$l$-dimensional vectors}\})$}{
      \uIf{$(\text{${x_i} = \mathit{in}'$ passes the type check})$}{
        $out \gets \runInterp(t', \mathit{in}')$\;
        \uIf{$\mathit{out} \neq \textsc{nil}$}{
            $\mathit{SummarySet}'(t, i) \gets \mathit{SummarySet}'(t, i) \cup (\mathit{in}, \mathit{out})$\;
            $\Pi \gets \Pi \cup \{out\}$\;
        }
      }
    }
  }
  \Return{$\mathit{SummarySet}'$}
}
\caption{Create the initial semantics summary by using the input states for parent term}
\label{alg:init-sem}
\end{algorithm}

==> algorithms/refine.tex <==

\begin{algorithm}
\Proc{$\algRefine(\mathit{prod}, \mathit{perm}, \mathit{sem}, E, \mathit{SummarySet})$}{
  $k \gets \text{number of child terms in $\mathit{prod}$}$\;

\For{$(\mathit{in}, t, \_) \in E$}{
  $S \gets \mathit{SummarySet}$\;
  % \jiangyichanged{--- CHANGE STARTS HERE ---}\;
  \While{$\top$}{
      $\xi \gets \top$\;
      \For{$i \gets \mathit{perm}(1 \dots k)$}{
        \For{$(\overline{{x_i}}, o) \in S(i)$}{
           \lIf{$o \neq \textsc{nil}$}{
             $\xi \gets \xi \land ({x_i} = \overline{{x_i}} \to y_i = o)$
           }
           \lElse{
             $\xi \gets \xi \land ({x_i} \neq \overline{{x_i}})$
           }
        }
      }
      $\mathit{model} \gets \algSolveSAT(\{\mathit{sem}.\phi \land \mathit{sem}.{x_0} = \mathit{in} \land \xi \})$\;
      $\mathit{found} \gets \bot$\;
      \If{$\mathit{model} \neq \textsc{nil}$}{
        \tcp{Program terminates on $\mathit{in}$}
        \For{$i \gets \mathit{perm}(1 \dots k+1)$}{
            % \tcp{${x_{k+1}}, y_{k+1}$ are for recursive call to $\semanticBrackets{\cdot}_{A}$}
            \lIf{$\overline{\mathit{perm}}(i) = k+1 \land (\lnot recursive(prod) \lor \lnot model(sem.\psi))$}{
              \textbf{break}
            }
            \lIf{$\overline{\mathit{perm}}(i) = k+1$}{$t' \gets t$}\lElse{$t' \gets t.child[i]$}
            $\mathit{in}' \gets model({x_i})$\;
            $\mathit{out}' \gets \runInterp(t', \mathbf{\overline{x_i}})$\; % JL TODO: Better naming for interpreter
            \lIf{$(\mathit{in}', \mathit{out}') \not\in S(i)$}{
              $found \gets \top$
            }
            $S(i) \gets S(i) \cup (\mathit{in}', \mathit{out}')$\;
        }
        
      }
      \If{$\lnot \mathit{found}$}{
         \tcp{The fixpoint shall be added to $\mathit{SummarySet}$}
         \For{$i \gets \mathit{perm}(1 \dots k+1)$}{
           $\mathit{SummarySet}(t, i) \gets \mathit{SummarySet}(t, i) \cup S(i)$\;
         }
         \Break
      }
    }
    
    % \jiangyichanged{--- CHANGE ENDS HERE ---}\;
  }  
  \Return{$\mathit{SummarySet}$}
}
\caption{Add missing input/output pairs for child terms (given the input states $\Sigma_{ex}$ to parent terms in $T$) to complete their summary sets}
\label{alg:refine}
\end{algorithm}


==> algorithms/sygus-grammar.tex <==

\begin{algorithm}
\Proc{$\algGenGrammar(\mathit{prod}, \mathit{perm}, f, \mathcal{T})$}{
  $A \mapsto \sigma(A_1, A_2, \dots, A_k) \gets \mathit{prod}$\;
  \eIf{$f$ is predicate function $\psi$}{
    $V \gets \{\text{all boolean variables in }y_1, y_2, \dots, y_k\}$\;
    $N \gets \{S\}$\;
    $\Sigma \gets \{\tok{and}, \tok{or}, \tok{not}\} \cup V$\;
    $P \gets \{S \mapsto S~\tok{and}~S,\; S \mapsto S~\tok{or}~S,\; S \mapsto \tok{not}~S\} \cup \{S \mapsto v \mid v \in V\}$\;
    \Return{$(N, \Sigma, S, P)$}
  }{
    \lIf{$f$ is $\phi_{rec}$}{$l \gets k + 1$}
    \lElse{$l \gets k$}

    \tcp{declare components of SyGuS grammar}
    $N \gets \{S, T, S_1, \dots, S_l\}$\;
    $\Sigma \gets \mathit{sig}(\mathcal{T}) \cup \{x_0, y_0, \dots, x_l, y_l\}$\;
    $\delta_0 \gets (S \mapsto \left(\bigwedge_{1 \le i \le l} x_i = S_i\right) \land (y_0=T))$\;
    $P \gets \{\delta_0\}$\;

    \tcp{$\mathit{vars}$ contain output variables of already evaluated terms}
    $\mathit{vars} \gets \emptyset$\;
    \For{$i \gets \mathit{perm}(1 \dots l)$}{
      \tcp{follow the evaluation order in $\mathit{perm}$}
      $P \gets P \cup \{S_i \mapsto v \mid v \in \mathit{vars}\} \cup \{S_i \mapsto x_0\}$\;
      $\mathit{vars} \gets \mathit{vars} \cup \{y_i\}$\;
    }
    $P \gets P \cup \{T \to \text{all $\tau$-typed expressions in $\mathcal{T}$ using $\{x_0\}\cup\mathit{vars}$} \}$\tcp*{$y_0$ is typed $\tau$}
    \Return{$(N, \Sigma, S, P)$}
  }
}
\caption{Generate SyGuS grammar for $\varphi$, $\phi_\mathit{rec}$, $\phi_\mathit{nonrec}$, or $\psi$}
\label{alg:sygus-grammar}
\end{algorithm}

==> algorithms/sygus.tex <==

\begin{algorithm}
% \Proc{$\algGenSygus(\mathit{prod}, \mathit{perm}, E, \mathit{funcs}, \mathit{SummarySet})$}
% {

%     $(A \mapsto \sigma(A_1,A_2,\dots,A_k)) \gets \mathit{prod}$\;
%     $\Gamma \gets \top$\;
%     \For{$(\mathit{in}, t, \mathit{out}) \in E$}{
%         \eIf{$\lnot \mathit{recursive}(\mathit{prod})$}{
%             $approx \gets \exists A_k. A_k \not\in \mathit{learnt}$\;
            
%             \If{approx}{
%                 $\mathit{SummarySet} \gets \algInitSem(\mathit{prod}, \mathit{perm}, t, \mathit{in}, \mathit{SummarySet}, \bot)$\;
%                 $\xi \gets \algApproxSummary(\mathit{prod}, \mathit{perm}, t, \mathit{SummarySet}, \bot, \top)$
%             }
%             \Else {
%                 $\xi \gets (\bigwedge_{i} \semanticBracketsWithNonterm{A_i}{t}{{x_i}^t} = y_i^t)$\tcp*{semantics already learnt}
%             }
%             $\varphi \gets \mathit{funcs}.\varphi$\;
%             $G \gets \algGenGrammar(\mathit{prod}, \mathit{perm}, \varphi, \mathcal{T})$\;
%             $\Gamma \gets \Gamma \land [
%               {x}_0^t = \mathit{in} \land \xi \land \varphi^G({x_0^t}, y_0^t, \dots, {x_k^t}, y_k^t) \to y_0^t = out
%             ]$\;
%         }{
%             \tcp{TODO: move to appendix?}
%             \tcp{Generate summaries}
%             $\mathit{SummarySet} \gets \algInitSem(\mathit{prod}, \mathit{perm}, t, \mathit{in}, \mathit{SummarySet}, \bot)$\;
%             $\mathit{SummarySet} \gets \algInitSem(\mathit{prod}, \mathit{perm}, t, \mathit{in}, \mathit{SummarySet}, \top)$\;

%             $\xi_\mathit{nonrec} \gets \algApproxSummary(\mathit{prod}, \mathit{perm}, t, \mathit{SummarySet}, \bot, \top)$\;
%             $\xi_\mathit{rec} \gets \algApproxSummary(\mathit{prod}, \mathit{perm}, t, \mathit{SummarySet}, \bot, \top)$\;
            
%             \tcp{Declare SyGuS functions ($\phi_{\mathit{rec}}$ and $\phi_{\mathit{nonrec}}$ are under theory $\mathcal{T}$)}
%             $\phi_{\mathit{rec}}, \phi_{\mathit{nonrec}}, \psi \gets \mathit{funcs}$\;
%             $G \gets \algGenGrammar(\mathit{prod}, \mathit{perm}, \phi_\mathit{rec}, \mathcal{T})$\;
%             $G' \gets \algGenGrammar(\mathit{prod}, \mathit{perm}, \phi_\mathit{nonrec}, \mathcal{T})$\;
%             $G'' \gets \algGenGrammar(\mathit{prod}, \mathit{perm}, \psi, \mathtt{bool})$\;
%             \tcp{${x_{\mathit{perm}(k+1)}^t}, y_{\mathit{perm}(k+1)}^t$ are input/output variables for the recursive call $\semanticBrackets{\cdot}_{A}$}
            
%             $\Phi_\mathit{rec} \gets \phi_\mathit{rec}^G(x_0^t, y_0^t, x_{\mathit{perm}(1)}^t, y_{\mathit{perm}(1)}^t, \dots,x_{\mathit{perm}(k+1)}^t, y_{\mathit{perm}(k+1)}^t)$\;
%             $\Phi_\mathit{nonrec} \gets \phi_\mathit{nonrec}^{G'}(x_0^t, y_0^t, x_{\mathit{perm}(1)}^t, y_{\mathit{perm}(1)}^t, \dots,x_{\mathit{perm}(k)}^t, y_{\mathit{perm}(k)}^t)$\;
            
%             \tcp{$\psi$ is under theory $\mathtt{bool}$}
%             $\Psi \gets \psi^{G''}(\text{all bools in I/O variables})$\;

%             \tcp{Generate SyGuS constraints}
%             $P \gets ({x_0^t}=\mathit{in} \land \lnot\Psi \land \xi_\mathit{nonrec} \land \Phi_\mathit{nonrec} \to y_0^t = out)$\;
%             $Q \gets ({x_0^t}=\mathit{in} \land \Psi \land \xi \land \Phi_\mathit{rec} \to y_0^t = out \land {x_0^t} \neq {x_{k+1}^t} \land ({x_{k+1}^t}, \textsc{nil}) \not\in SummarySet(t, k+1))$\;
%             $\Gamma \gets \Gamma \land (P \land Q)$\;
%         }
%     }
%     \Return{$\Gamma$}
% }
\Proc{$\algSygus(\mathit{prod}, E)$}{
    \tcp{The SyGuS grammars follow \cref{eqn:semantic-constraint-condition}}
    $\Gamma \gets \text{SyGuS grammars used for semantics of $\mathit{prod}$}$\;
    $m \gets \algSolveSygus(\Gamma)$\;
    
    \tcp{Extract solution}
    \lIf{$\lnot recursive(prod)$}{
    $\phi \gets m(\varphi)$
    }
    \lElse{
    $\phi \gets [m(\psi) \to m(\phi_\mathit{rec}) \land \lnot m(\psi) \to m(\phi_\mathit{nonrec})]$
    }
    \Return{$\{m, \phi\}$}
}
\caption{Find a candidate semantics for a certain $\mathit{prod}$ using SyGuS} \label{alg:sygus}
\end{algorithm}




==> algorithms/syn-all.tex <==
\begin{algorithm}
\Glob{
  $\mathit{learnt} \gets \emptyset$ \tcp*{Stores all synthesized semantics}
}
\Proc{$\algAll\left(grammar\right)$}{
  $(N,\Sigma,S,P) \gets \mathit{grammar}$\tcp*{$P$ contains ``\texttt{recursive}'' tag}
  \tcp{\jiangyi{We might substitute the next line with weak topological order later.}}
  \For{$\mathit{prod} \in P$}{
    \lIf{$\mathit{recursive}(\mathit{prod})$}{$\mathit{perm} \gets \{0, 1, \dots, k+1\}$}
    \lElse{$\mathit{perm} \gets \{0, 1, \dots, k\}$}
    $\mathit{sem} \gets \textsc{nil}$\;
    \Repeat{$\mathit{sem} \neq \textsc{nil} \lor \text{no next permutation for $\mathit{perm}$}$}{
        $\mathit{sem} \gets \algSingle(\mathit{prod}, \mathit{perm})$\;
        $\mathit{perm} \gets \text{next permutation}$\;
    }
    \Assert{$\mathit{sem} \neq \textsc{nil}$}
    $\mathit{learnt}[\mathit{prod}] \gets \mathit{sem}$
  }
  \Return{$\mathit{learnt}$}
}
\caption{Synthesize all semantics
}
\label{alg:syn-all}
\end{algorithm}

==> algorithms/syn-single.tex <==
\begin{algorithm}
\Proc{$\algSingle(\mathit{prod}, \mathit{perm})$}{
  $E \gets \emptyset$ \tcp*{Example set}
  $\mathit{SummarySet} \gets \text{empty mapping}$ \tcp*{Maps $(\mathit{term}, \#\mathit{child})$ to I/O pairs}
  \While{$\mathit{\top}$}{
    \tcp{TODO: define funcs}
    $\mathit{sem} \gets \mathit{\algSygus}(\mathit{prod}, \mathit{perm}, E, \mathit{funcs}, \mathit{SummarySet})$\;
    \lIf{$\mathit{sem} = \textsc{nil}$}{\Return{\textsc{nil}}}
    $\mathit{SummarySet'} \gets \algRefine(\mathit{prod}, \mathit{perm}, \mathit{sem}, E, \mathit{SummarySet})$\;
    \eIf{$\mathit{SummarySet'} = \mathit{SummarySet}$}{
      $E'\gets \textsc{FuzzTermsAndInputs()}$\;
      $(\mathit{t}, \mathit{in}, \mathit{SummarySet}'') \gets \algVerify(\mathit{prod}, \mathit{perm}, \mathit{sem}, E, E', \mathit{SummarySet}')$\;
      $\mathit{SummarySet} \gets \mathit{SummarySet''}$\;
      \eIf{$\mathit{t} = \textsc{nil}$}{
        \Return{$\mathit{sem}$}
      } {
        $\mathit{out} \gets \runInterp(t, \mathit{in})$\;
        $E \gets E \cup (\mathit{in}, t, \mathit{out})$\;
      }
    } {
      $\mathit{SummarySet} \gets \mathit{SummarySet'}$\;
    }
  }
}
  \caption{Synthesize semantics for a single term with CEGIS
  } \label{alg:syn-single}

\end{algorithm}


==> sections/4-alt-algorithm-optimization.tex <==
\subsection{Optimization for multi-output semantic rules}\label{sec:algorithm:optimization}

Algorithm~\ref{alg:syn-all} generally works for all semantic rules, regardless of the number of inputs and outputs (e.g., when there're multiple outputs, output variables $\{y_i\}$ become vectors). However, initial experiments have shown that empirically, SyGuS calls cannot terminate within our time limit if the search space is too big due to the number of output variables. Consider line 12 of Algorithm~\ref{alg:sygus}, if every argument $x_i$ and $y_i$ of $\varphi^G$ is a two-dimensional vector, then the start rule generated on line 14 of Algorithm~\ref{alg:sygus-grammar} will become twice the size as before, since vector equalities have to be converted into conjunction of scalar equalities for SyGuS solver compatibility. This, in turn, at least squares the size of search space.

To alleviate this problem, we divide the SyGuS problems into sub-problems, each containing all inputs but only contains one component of output $y_0$. After solving the sub-problems, we check if the dataflow relations match (assignments to $x_1, x_2, \dots$ are equivalent), and regenerates whenever a mismatch happens.

\input{algorithms/multi-output}

The pseudo-code is shown in Algorithm~\ref{alg:sygus-multi}.
The components of an output vector $y_0$ are denoted as $y_0^0, y_0^1, y_0^2, \dots$, and for each SyGuS function $f(x_0, y_0, \dots, x_k, y_k)$, a partial function $f^i(x_0, y_0^i, \dots, x_k, y_k)$ is created for output component $y_0^{i}$ (line 7).
For each partial function, we generate the SyGuS sub-problem by invoking $\algGenSygus$ (line 8).
Then it tries to find dataflow inconsistencies between partial functions (line 11--15).
If no such inconsistency is found, partial functions are merged together to form the candidate semantics.
Otherwise, SMT solver is called to find assignments to arguments that witness the dataflow inconsistency (line 20--21), which are then used to prevent the current functions from being synthesized again (line 22).

But why breaking the function into multiple partial functions with scalar outputs makes the synthesis faster?
Intuitively speaking, it uses another CEGIS-style loop to alleviate the workload for every solver call.
Before this optimization, the SyGuS solver has to find the correct expression for \emph{every} output variable before returning a candidate function.
For ease of computation, we do not consider the search space for data flow variables ($x_1,x_2,\dots$) as they are of constant size.
If the size of expression search space for one output component is $S$, and the output has $k$ components, then for synthesizing the function, a search space of size $O(S^k)$ will have to be iterated.
However, when using Algorithm~\ref{alg:sygus-multi}, only one correct term needs to be synthesized (for one output component) in every solver call.
In one iteration of the CEGIS loop (line 5--26 in Algorithm~\ref{alg:sygus-multi}), the total size of all search space is reduced to $O(kS)=\log O(S^k)$.
The time spent on SyGuS solvers is reduced logarithmically.

==> sections/old-algorithm.tex <==
\section{Algorithm} \label{sec:algorithm}

To synthesize the formal semantics, we utilized a well-known approach called CounterExample-Guided Inductive Synthesis (CEGIS). For every production rule, we first synthesize a candidate semantic rule, and then try to find a counterexample that falsifies it, i.e., exposing a different behavior than the oracle interpreter. The details of the CEGIS loop will be provided later. The main difference between our approach and the standard CEGIS loop is in the use of approximated semantics.
%\charlie{I would say CEGIS is a class of algorithms for which this is one of. I think it's best practice to explicitly describe our method rather than assuming the reader knows the ``typical'' approach and describing the differences.}

It is possible that the semantic function that we are currently synthesizing depends on another semantic function that is currently unknown. There are two possible cases of this: either we have not synthesized the referred semantic function yet, or the current semantic function is recursively defined. Consider the semantic function of \texttt{while} in IMP (\jiangyi{TODO: list the grammar of while; paraphrase}): if the loop condition evaluates to TRUE, the semantic function of \texttt{while} recursively calls itself.
%\charlie{Yes, use an example that you can weave through the description of the algorithms. This will greatly aid a reader. This example could even be introduced in an earlier section and used throughout the paper to describe technical definitions.}

Input/output examples are used to model the behavior of currently unknown semantic functions. For an unknown semantic function $\semanticBracketsWithNonterm{A}{t_i}{\mathbf{x_i}}$ of a child term $t_i$, it can be approximated with a \emph{summary set} $\{(\mathbf{x_i^k}, y_i^k) \mid k\}$, where $y_i^k = I_A(t_i, \mathbf{x_i^k})$. If $y_i$ is the evaluated value of $t_i$ under $x_i$, we can then denote such an approximation as $\bigwedge_{k} \mathbf{x_i} = \mathbf{x_i^k} \to y_i = y_i^k$. Such an approximation is defined as a \emph{summary}.

However, the summary can be inadequate when $\mathbf{x_i}$ does not equal to any known input examples, i.e., $\mathbf{x_i} \not\in \{\mathbf{x_i^k} \mid k\}$, leading to wrong candidate semantics. Algorithm~\ref{alg:refine} is thus created, where $\algRefine$ adds new elements into the input/output example set to cover new cases. After new input/output examples are generated, the new summary $\bigwedge_{k} \mathbf{x_i} = \mathbf{x_i^k} \to y_i = y_i^k$ is then constructed in the function $\algInitSem$ (Algorithm~\ref{alg:init-sem}).
\charlie{It's unclear which algorith / part of the algorithms the above describes. I would assume that this would describe \ref{alg:syn-all}. But make this explicit. If some part is done in a different algorithm, mention which algorithm that is (like you did here).}

\jiangyi{Define what is an \emph{accurate} summary that covers every input?}



\subsection{Overview\label{sec:algorithm:overview}} 
% \charlie{I think this will be addressed by my suggested changes to Section 3. I think this ``Assumption on dataflow'' is about order of evaluation of sub-terms. I think we have an algorithm that operates from a given fixed order of evaluation/dataflow. Then a function that in parallel tries all possible orders of evaluation. Then simply returns the first one to succeed. Does the algorithm as currently described allowed to return failure? I.e. no such semantics for the given order of evaluation satisfies the example set? If this isn't clear / doesn't work after updating section 3, we'll revisit this.
% }
The algorithm starts with Algorithm~\ref{alg:syn-all}, where we synthesize the semantics for each production rule of the regular tree grammar by invoking Algorithm~\ref{alg:syn-single} (line 5, line 10). If a solution is found, it will be stored into the map $\mathit{learnt}$ (line 13) and utilized for upcoming synthesis.

To account for the evaluation orders (defined in Section~\ref{sec:problem-definition:semantics}), we start with the identity permutation (line 6--7 in Algorithm~\ref{alg:syn-all}) and then enumerate all possible permutations $p$ for each production rule (line 11). For each $p$, the algorithm tries to synthesize a semantics using $p$ as the evaluation order. If there's no solution under such a $p$, it continues enumerating new permutations until a solution is found (line 12).


\subsection{CEGIS loop\label{sec:algorithm:cegis}}

Algorithm~\ref{alg:syn-single} contains the main CEGIS loop (line 4--18). Line 5 calls $\algSygus$ to generate a candidate. Line 7 completes the summary. After that, lines 9--10 try to verify the candidate semantics. If the verification passes (line 12) then the loop halts. Otherwise, the counterexample term and input will be added to the example set $E$ (line 15--16) and used for synthesis in the next rounds.

\input{algorithms/syn-all}
\input{algorithms/syn-single}

\subsection{Transformation into a \textsc{SyGuS} problem\label{sec:algorithm:sygus}}

Algorithm~\ref{alg:sygus} uses the current example set $E$ to create a candidate definition of semantic function by utilizing a SyGuS solver. We first introduce how we generate grammars used for SyGuS functions, and then discuss the creation of SyGuS function constraints.

\paragraph{Grammars for SyGuS Problems}

\input{algorithms/sygus-grammar}

To synthesize the function $\varphi$ (or $\phi_\mathit{rec},\phi_\mathit{nonrec}$ and $\psi$ in the recursive case) under SyGuS, a grammar for each function is required. Algorithm~\ref{alg:sygus-grammar} generates the grammar based on function type, theory and the evaluation order (provided as a permutation $\mathit{perm}$).

For the predicate function $\psi$, the grammar contains all boolean variables and their boolean combinations. For other functions, the grammar contains assignments to each child term's inputs ($x_{\mathit{perm}(1)},\dots,x_{\mathit{perm}(l)}$, considering evaluation order) and the final output expression $y_0 = \cdot$.

\paragraph{SyGuS Function Constraints}

\input{algorithms/sygus}

For each example in $E$ (line 4), the algorithm creates SyGuS constraints that describes how should the semantics behave. Given a specific example $(in, t, out) \in E$, different constraints are created for for non-recursive and recursive semantics.

The non-recursive case is rather straightforward. Suppose that the current production rule is $prod = (A \mapsto \sigma(A_1, \dots, A_k))$. Recall that the current semantic function $\semanticBrackets{t}_{A}$ may depend on semantics of child terms, which can be undefined. In the case where undefined child semantics exist (line 7), Algorithm~\ref{alg:init-sem} is invoked (line 8--9) to create an initial summary and construct an SMT formula consisting the input/output pairs in the summary. Otherwise, the semantic functions of child terms will be directly used (line 11).
The function $\varphi$ to be synthesized is the candidate semantics that relates root input/output variables ($x_0, y_0$) and those of $t$'s child terms ($x_1,y_1,x_2,y_2,\dots$) together. An example of $\varphi$ has already been provided in Section~\ref{sec:example}, where it corresponds to $x_1 = x_0 \land x_2 = y_1 \land y_0 = y_2$ in the final semantics.

For the recursive case, however, three functions, $\phi_{rec}$, $\phi_{nonrec}$ and $\psi$, need to be synthesized. The three functions will then form two semantic rules. As the semantic function itself is recursively invoked, we have to use summaries when synthesizing it, because it exact semantics are still unknown at this time. We first create the initial summaries on line 15--18. $\phi_{rec}$ and $\phi_{nonrec}$ are declared on line 22--23. Line 24 declares $\psi$, the recursion guard: when it evaluates to $\bot$, \textsc{NonRec} in Equation~\ref{eqn:rec-rule-1} will be applied (corresponds to $P$ on line 25); when it is $\top$, the rule \textsc{Rec} in Equation~\ref{eqn:rec-rule-2} will be applied instead (corresponds to $Q$ on line 26).

\begin{equation}
\label{eqn:rec-rule-1}
\inferrule{
    \bigwedge_{i \gets \mathit{perm}(1 \dots k)}\semanticBracketsWithNonterm{A_i}{t_i}{{x_i}} = y_i \\
    \lnot\psi \\ \phi_{nonrec}({x_0}, y_0, \dots, {x_k}, y_k)
}{\semanticBracketsWithNonterm{A}{t}{{x_0}} = y_0} \textsc{NonRec}
\end{equation}
\begin{equation}
\label{eqn:rec-rule-2}
\inferrule{
    \bigwedge_{i \gets \mathit{perm}(1 \dots k)}\semanticBracketsWithNonterm{A_i}{t_i}{{x_i}} = y_i \\
    \semanticBracketsWithNonterm{A}{t}{{x_{\mathit{perm}(k+1)}}} = y_{\mathit{perm}(k+1)} \\
    \psi \\ \phi_{rec}({x_0}, y_0, \dots, {x_{k+1}}, y_{k+1})
}{\semanticBracketsWithNonterm{A}{t}{{x_0}} = y_0} \textsc{Rec}
\end{equation}

After adding constraints for every example in $E$,the algorithm calls the SyGuS solver to synthesize $\phi_{rec}$, $\phi_{nonrec}$ and $\psi$ (line 28). Then, the solution is extracted from the model and returned (line 29--31). 

\subsection{Summary for Child Terms\label{sec:algorithm:summary}}

Algorithm~\ref{alg:init-sem}, Algorithm~\ref{alg:approx-summary} and Algorithm~\ref{alg:refine} are related to the creation of initial summary sets, which are then used as an approximation for unknown semantics.

\input{algorithms/init-sem}

Algorithm~\ref{alg:init-sem} initializes the summary set using the input value of parent term $t$. For each child term (line 10) or the recursive call of semantic function (line 7--8), we try to assembly the argument vector $\mathbf{x_i}$ with values in $\Pi$ (line 12--13). We also try to directly assign values in the summary set to the argument vector (line 13). If running the child term (with argument vector $in$) terminates normally, the input/output pair $(in, out)$ will then be recorded in the summary set (line 19). Last, the evaluation result $out$ is added to the set of values $\Pi$.

\input{algorithms/approx}

Algorithm~\ref{alg:approx-summary} creates an SMT formula that simulates the behavior of a certain child term using the input/output pairs summary set. It just enumerates each child term by the evaluation order (line 4), and add input/output mappings from the summary set to the formula (line 7--9).

\input{algorithms/refine}

Algorithm~\ref{alg:refine} attempts to find new input/output examples that is not covered by the current summary. It starts by looping through all examples in $E$ (line 2--3). For each example $(in, t, _) \in E$, a fixpoint algorithm is then used to complete the summary for each child.

In each iteration (line 3) we use the definition of candidate semantics $cand$ to populated input/output values to the child terms, which is done with SMT solvers on line 11. 
Then, the algorithm iterates through all child terms (line 14) and extract the input value for each term (line 18). If such an input example is not previously known in the summary set (line 24). If no such example can be found, the summary set is returned unchanged.


\subsection{Validation of Candidate Semantics\label{sec:algorithm:validation}}

Algorithm~\ref{alg:verify} validates the candidate semantic function by finding counterexamples with a SAT solver. Due to the fact that the interpreter is treated as a closed-box, we cannot use techniques like symbolic execution to get an accurate oracle for verification. Instead, we have to rely on example terms and inputs to model the behavior of the interpreter. The more examples we used, the better the model of interpreter will be. Thus, a comprehensive bank of possible examples, $E'$, shall be passed in. Algorithm~\ref{alg:verify} check the correctness of the candidate semantics by iterating through $E \cup E'$ (line 4). If the candidate failed on the given examples, the the validation fails and returns the term, input example, and refined summary set (line 13). Otherwise, $(\textsc{Nil}, \textsc{Nil}, \mathit{SummarySet}')$ is returned.

\input{algorithms/verify}

\subsection{Correctness\label{sec:algorithm:correctness}}

\jiangyi{TODO: theorems of correctness; better captions for algorithms}

We show that the main algorithm (Algorithm~\ref{alg:syn-single}) is able to synthesize a set of semantics that is correct regarding Definition~??.

\begin{theorem}[Algorithm~\ref{alg:syn-single} is sound and complete]For any grammar $G = \tuple{N,\Sigma,S,\delta,\mathcal{T},\theta,\tau}$ and interpreter $I$, $\algAll$ terminates and returns a learned semantics $\mathit{learnt}$ such that for every production rule $p \in \delta$ of $G$, the learned semantics of $p$ is sound with respect to the terms and inputs ($\mathit{TermBank}$ and $\mathit{Inputs}$) produced by the interpreter $I$.

Formally, for every production rule $p$ that starts with nonterminal $A \in N$:
\[t \in \mathit{TermBank}[p] \land \sigma \in \mathit{Inputs}[p] \Rightarrow \semanticBracketsWithNonterm{A}{t}{\sigma} = I_A(t,\sigma)
\]
\end{theorem}

\begin{proof}
    Algorithm~\ref{alg:syn-single} only returns on line 12, where $cex = \textsc{nil}$ holds. According to Algorithm~\ref{alg:verify}, $(\textsc{nil}, \textsc{nil})$ may be returned only when the loop on line 4--13 of Algorithm~\ref{alg:verify} does not find any counterexample term. We assume that the contrary holds, i.e., $\semanticBracketsWithNonterm{A}{t}{\sigma} \neq I_A(t,\sigma)$. In this case, the satisfiability check on line 12 will pass (see lemmas later) and a counterexample will be returned. Since no counterexample can be found, we conclude that the assumption is wrong, and $\semanticBracketsWithNonterm{A}{t}{\sigma} = I_A(t,\sigma)$.
\end{proof}

\begin{lemma}[CEGIS loop makes progress]
    Any candidate $\mathit{sem}$ found in a previous round of Algorithm~\ref{alg:syn-single} will either be the final solution, or be rejected in upcoming rounds.
\end{lemma}
\begin{proof}
    We show that for a certain candidate $\mathit{sem}$, it is eventually passed to \algVerify for counterexample search.
    For a certain iteration, it either passes through line 6--9 and reaches line 10 directly, or reaches line 18 (when new items are added to the summary) and starts another iteration.

     First, we have to prove that the latter case eventually happens for a certain $\mathit{sem}$, i.e., \algRefine saturates in the end. \jiangyi{TODOTODOTODO}

    Then we show that the lemma holds when a new SyGuS solver call happens.

    \paragraph{$\mathit{prod}$ is non-recursive}
    For the case where $\mathit{prod}$ is non-recursive, given that a counterexample has already be found, we know ${x_0}=\mathit{in} \land \xi \land \varphi \land y_0 \neq \mathit{out}$ holds for the counterexample $(\mathit{in}, \mathit{out})$ (line 12--13 of \algVerify).
    If the production rule is non-recursive, then $\xi$ in \algSygus is defined the same way as $\xi$ in \algVerify. The counterexample $(\mathit{in}, \mathit{out})$ can never satisfy line 14 of Algorithm~\ref{alg:sygus}, since it satisfies ${x_0}=\mathit{in} \land \xi \land \varphi \land y_0 \neq \mathit{out}$, which can be rewritten as $\lnot ({x_0}=\mathit{in} \land \xi \land \varphi \to y_0 = \mathit{out})$

    \paragraph{$\mathit{prod}$ is recursive}
    For the recursive case the proof is more complex: one has to show that $\lnot (P \land Q)$ always holds (under the context of line 23 of \algSygus). We can see that for recursive production rules, $\phi$ is defined as line 24 in \algSygus. If we plug such a $\phi$ into $\mathit{sem}.\phi$ on line 12 of \algVerify, we get:

    \[\xi \land {x_0}=\mathit{in} \land y_0 \neq \mathit{out} \land \psi \to \phi_\mathit{rec} \land \lnot\psi \to \phi_\mathit{nonrec}\]

    We then show that: the formula above (denoted as $F$) implies $\lnot (P \land Q)$, which means that the counterexample rejects $\mathit{sem}.\phi$ in the next round.
    To show that $F \Rightarrow \lnot (P \land Q)$, one must show that either $F \Rightarrow \lnot P$ or $F \Rightarrow \lnot Q$.

    We first prove $F \Rightarrow \lnot P$ for the case where $\lnot \psi$ holds (excluded middle). Note that $\xi=\xi_\mathit{rec}$(line 11 of Algorithm~\ref{alg:verify}), so $\xi=\xi_\mathit{rec} \Rightarrow \xi_\mathit{nonrec}$ (\jiangyichanged{LEMMA: superset relations of $\xi$'s}). Therefore, the formula above implies $\lnot P$.

    Then we show that $F \Rightarrow \lnot Q$ for the case where $\psi$ holds.
    Proving $F \Rightarrow \lnot Q$ can be divided into two subgoals:
    (1) $F \Rightarrow {x_0}=\mathit{in} \land \psi \land \xi_\mathit{rec} \land \phi_\mathit{rec} \land y_0 \neq \mathit{out}$;
    (2) $F \Rightarrow {x_0}=\mathit{in} \land \psi \land \xi_\mathit{rec} \land \phi_\mathit{rec} \land [{x_0} = {x_{k+1}} \lor ({x_{k+1}}, \textsc{nil}) \in \mathit{SummarySet}(t, k+1)]$.
    As (1) can be easily proven, we focus on the subgoal (2).
    For subgoal (2), case analysis introduced a premise $y_0 = \mathit{out}$, which contradicts with $F$.
    Hence, this subgoal can never appear.

    Therefore, the candidate generated in a previous round can never become the candidate again in \algSygus.
\end{proof}

\begin{lemma}[Correctness of using summary]
    For Algorithm~\ref{alg:verify}, the satisfiability check on line 14 passes iff $\dots$ \jiangyi{TODO}
\end{lemma}

==> semantics/bitvec.tex <==
\begin{mathpar}
    \inferrule{\xspace}{\semanticBracketsUsing{\tok{0x00}}{\sigma}=\mathtt{00000000}}~\textsc{BvZero} \and
    \inferrule{\xspace}{\semanticBracketsUsing{\tok{0x01}}{\sigma}=\mathtt{00000001}}~\textsc{BvOne} \and
    \inferrule{\semanticBracketsUsing{b_1}{\sigma} = v_1 \\ \semanticBracketsUsing{b_2}{\sigma} = v_2}{\semanticBracketsUsing{(\tok{bvand}~b_1~b_2)}{\sigma}=v_1 \mathbin{\&} v_2}~\textsc{BvAnd} \and
    \inferrule{\semanticBracketsUsing{b_1}{\sigma} = v_1 \\ \semanticBracketsUsing{b_2}{\sigma} = v_2}{\semanticBracketsUsing{(\tok{bvor}~b_1~b_2)}{\sigma}=v_1 \mathbin{|} v_2}~\textsc{BvOr} \and
    \inferrule{\semanticBracketsUsing{b}{\sigma} = v}{\semanticBracketsUsing{(\tok{bvnot}~b)}{\sigma}=\mathord{\sim} v}~\textsc{BvNot} \and
    \inferrule{\semanticBracketsUsing{b}{\sigma} = v}{\semanticBracketsUsing{(\tok{bvneg}~b)}{\sigma}=(\mathord{\sim} v) +\mathtt{00000001}}~\textsc{BvNeg} \and
    \inferrule{\semanticBracketsUsing{b_1}{\sigma} = v_1 \\ \semanticBracketsUsing{b_2}{\sigma} = v_2}{\semanticBracketsUsing{(\tok{bvadd}~b_1~b_2)}{\sigma}=v_1 \mathbin{+} v_2}~\textsc{BvAdd} \and
\end{mathpar}

==> semantics/lang-signatures.tex <==
\begin{figure}[h!]
    \centering
    \fbox{\begin{minipage}[t][6cm][t]{0.45\textwidth}
        \textbf{\textsc{Currency}}\\
        Language Grammar
        \begin{align*}
            S &\Coloneqq S \mathbin{\tok{+}} S \mid S \mathbin{\tok{+}} S \mid S \mathbin{\tok{\times}} K \\
              &\mid \tok{usd}~K \mid \tok{cny}~K \mid \tok{jpy}~K\\
            K &\Coloneqq \tok{x} \mid \tok{0} \mid \tok{1} \mid \tok{2} \mid \tok{4} \mid \tok{8} \\
              &\mid \tok{16} \mid \tok{32} \mid \tok{64} \mid K \mathbin{\tok{+_{K}}} K
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_S&: \mcL\left(S\right) \times \ZZ \to \ZZ\\
        \semanticBrackets{\cdot}_K&: \mcL\left(K\right) \times \ZZ \to \ZZ\\
        \end{align*}
    \end{minipage}}
    \hspace*{0.01\linewidth}
    \fbox{\begin{minipage}[t][6cm][t]{0.43\textwidth}
        \textbf{\textsc{Imp}}\\
        Language Grammar
        \begin{align*}
        S &\Coloneqq \tok{x \coloneqq}~E \mid \tok{y \coloneqq}~E \mid S~\tok{;}~S \mid \tok{ite}~B~S~S \\
        &\mid \tok{while}~B~S \mid \tok{do\_while}~S~B \\
        E &\Coloneqq \tok{0} \mid \tok{1} \mid \tok{x} \mid \tok{y} \mid E \mathbin{\tok{+}} E \mid E \mathbin{\tok{-}} E \\
        B &\Coloneqq \tok{t} \mid \tok{f} \mid \tok{not}~B \mid \tok{and}~B~B \\
        &\mid \tok{or}~B~B \mid E \mathbin{\tok{<}} E
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_S&: \mathcal{L}\left(S\right) \to \ZZ^2 \to \ZZ^2\\
        \semanticBrackets{\cdot}_E&: \mathcal{L}\left(E\right) \to \ZZ^2 \to \ZZ^2\\
        \semanticBrackets{\cdot}_B&: \mathcal{L}\left(B\right) \to \ZZ^2 \to \mathtt{bool}
        \end{align*}
    \end{minipage}}%
    
    \vspace*{0.5em}
    
    \fbox{\begin{minipage}[t][4cm][t]{0.45\textwidth}
        \textbf{\textsc{LinAlg}}\\
        Language Grammar
        \begin{align*}
            M &\Coloneqq M \tok{\times} M \mid \tok{x} \mid \tok{transpose}~M \\
            I &\Coloneqq \tok{0} \mid \tok{1} \mid I \mathbin{\tok{+}} I \mid \tok{det}~M \mid \tok{trace}~M
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_M&: \mathcal{L}\left(M\right) \to \ZZ^{2 \times 2} \to \ZZ^{2 \times 2}\\
        \semanticBrackets{\cdot}_I&: \mathcal{L}\left(I\right) \to \ZZ^{2 \times 2} \to \ZZ
        \end{align*}
    \end{minipage}}
    \hspace*{0.01\linewidth}
    \fbox{\begin{minipage}[t][4cm][t]{0.43\textwidth}
        \textbf{\textsc{Diff}}\\ \\
        Language Grammar
        \begin{align*}
            E &\Coloneqq \tok{0} \mid \tok{1} \mid \tok{2} \mid \tok{x} \mid \tok{+}
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_M&: \mathcal{L}\left(M\right) \to \ZZ^{2 \times 2} \to \ZZ^{2 \times 2}\\
        \semanticBrackets{\cdot}_I&: \mathcal{L}\left(I\right) \to \ZZ^{2 \times 2} \to \ZZ
        \end{align*}
    \end{minipage}}

    \vspace*{0.5em}

    \fbox{\begin{minipage}{0.45\textwidth}
        \textbf{\textsc{RegEx}}\\
        Language Grammar
        \begin{align*}
            S &\Coloneqq \tok{eval}~E\\
            E &\Coloneqq \tok{\epsilon} \mid \tok{\phi} \mid \tok{a} \mid \tok{b} \mid \tok{?}
                \mid E \mathbin{\tok{+}} E \mid E \mathbin{\tok{\cdot}} E \mid E^{\tok{*}}
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_S&: \mathcal{L}\left(S\right) \to \{\tok{a},\tok{b},\dots,\epsilon\}^k \to \mathtt{bool}\\
        \semanticBrackets{\cdot}_E&: \mathcal{L}\left(E\right) \to \{\tok{a},\tok{b},\dots,\epsilon\}^k \to \mathtt{bool}^{(k+1)^2}
        \end{align*}
    \end{minipage}}
    \hspace*{0.01\linewidth}
    \fbox{\begin{minipage}{0.43\textwidth}
        \textbf{\textsc{RegExSimp}}\\
        Language Grammar
        \begin{align*}
            S &\Coloneqq \tok{eval}~E\\
            E &\Coloneqq \tok{\epsilon} \mid \tok{\phi} \mid \tok{a} \mid \tok{b} \mid \tok{?}
                \mid E \mathbin{\tok{+}} E \mid E \mathbin{\tok{\cdot}} E \mid E^{\tok{*}}
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_S&: \mathcal{L}\left(S\right) \to \{\tok{a},\tok{b},\dots,\epsilon\}^k \to \mathtt{bool}\\
        \semanticBrackets{\cdot}_E&: \mathcal{L}\left(E\right) \to \{\tok{a},\tok{b},\dots,\epsilon\}^k \to \mathtt{bool}^{p}\\
        p &= (k+1) k / 2 + 1
        \end{align*}
    \end{minipage}}

    \vspace*{0.5em}

    \fbox{\begin{minipage}[t][4cm][t]{0.45\textwidth}
        \textbf{\textsc{BinOp}}\\
        Language Grammar
        \begin{align*}
            S &\Coloneqq \tok{count}~N \mid \tok{bin2dec}~M \\
            N &\Coloneqq \tok{concat}~N~B \mid \tok{atom}~B \\
            M &\Coloneqq \tok{concat'}~M~B \mid \tok{atom'}~B \\
            B &\Coloneqq \tok{0} \mid \tok{1} \mid \tok{x}
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_A&: \mcL\left(A\right) \times \mathtt{bool} \to \ZZ (A \in \{S,N,M,B\})\\
        \end{align*}
    \end{minipage}}
    \hspace*{0.01\linewidth}
    \fbox{\begin{minipage}[t][4cm][t]{0.43\textwidth}
        \textbf{\textsc{BvExpr}}\\
        Language Grammar
        \begin{align*}
        E &\Coloneqq \tok{0} \mid \tok{1} \mid \tok{x} \mid \tok{y} 
        \mid \tok{bvand}~E~E \\
        & \mid \tok{bvor}~E~E \mid \tok{bvnot}~E \\
        &\mid \tok{bvadd}~E~E \mid \tok{bvneg}~E~E \mid \tok{lowbit}~E
        \end{align*}
        Signature of semantic functions
        \begin{align*}
        \semanticBrackets{\cdot}_E&: \mathcal{L}\left(E\right) \to (\mathtt{u32}, \mathtt{u32}) \to \mathtt{u32}
        \end{align*}
    \end{minipage}}
    
    \caption{Languages used for evaluation}
    \label{fig:dataset}
\end{figure}
